A Tool for In-depth Analysis of Code Execution Reasoning of Large Language Models

Code Executing Reasoning is becoming a new non-functional metric that assesses the ability of large language models (LLMs) in programming tasks. State-of-the-art frameworks (CodeMind or REval) and benchmarks (CruxEval) usually focus on LLM's prediction of a given code's input/output or intermediate variable states/values on limited programs. However, there is no tool for more in-depth analysis of the results. Without such a tool, the observations about LLM's code execution reasoning cannot be generalized to more datasets, preventing the research community and practitioners from devising the next generation of LLMs with better code execution reasoning abilities. This paper introduces ExeRScope, a series of tools and heuristics to analyze the result of code execution reasoning frameworks to understand better the impact of code properties in the studied benchmarks on the code execution reasoning. With such tooling, analysis can be generalized to code with similar properties without the urgent need to design more benchmarks, which is a cumbersome effort.

==> listing/icl_example.tex <==
\begin{lstlisting}[style=stylewithcommentPy]
@@Consider the following code:@@
def sum_of_integer(N, A, B):
   sum_1 = 0
   for i in range(1,N+1):
       sum_order = 0
       i_str = str(i)
       n = len(i_str)
       for j in range(0,n):
           sum_order += int(i_str[j])
       if A <= sum_order <= B:
           sum_1 += i
   return sum_1
@@[Question]@@
What would be the |return| value of `sum_of_integer(20, 2, 5)`
@@[Answer]@@
The variable N, variable A |and| variable B are initialized 
to 20, 2,|and| 5, respectively. variable sum_1 |is| initialized
to 0, which will be used to accumulate the |sum| of numbers 
meeting the condition. The code then enters a loop that 
iterates |from| 1 to N (inclusive), meaning it will consider
numbers |from| 1 to 20. For each number i |in| this |range|, it 
calculates the |sum| of its digits |and| stores it |in|
sum_order. The code checks |if| sum_order |is| within the |range|
[A, B], which |is| [2, 5] |in| this case. If it |is|, it adds 
the current number i to sum_1. The condition |is| met when 
i |is| 2,3,4,5,11,12,13,14 |and| 20. After the loop finishes,
the code prints the final value of sum_1, which |is| 84.
@@[Output]@@
84
\end{lstlisting}

==> tables/er.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Performance of subject LLMs in execution reasoning measured by $R_{ER}$}
\label{tab:er}
\vspace{-10pt}
\centering
\scalebox{0.61}{
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|cccccc|}
\hline
\multirow{2}{*}{\textbf{Dataset}} &
  \multirow{2}{*}{\textbf{\#Subjects}} &
  \multicolumn{6}{c|}{\textbf{Subject LLMs}} \\ \cline{3-8} 
 &
   &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CodeLlama\\ (Inst-34b)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DeepSeek-Coder\\ (Inst-33b)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Semcoder-S\\ (6.7b)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}StarCoder2\\ (15b)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Gemini-1.5-\\ Pro\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}GPT-4-\\ Turbo\end{tabular}} \\ \hline
\textbf{Avatar} &
  86 &
  \multicolumn{1}{c|}{23.26\%} &
  \multicolumn{1}{c|}{41.86\%} &
  \multicolumn{1}{c|}{30.23\%} &
  \multicolumn{1}{c|}{32.56\%} &
  \multicolumn{1}{c|}{54.65\%} &
  61.63\% \\ \hline
\textbf{ClassEval} &
  400 &
  \multicolumn{1}{c|}{43.50\%} &
  \multicolumn{1}{c|}{65.00\%} &
  \multicolumn{1}{c|}{61.60\%} &
  \multicolumn{1}{c|}{55.25\%} &
  \multicolumn{1}{c|}{74.00\%} &
  77.50\% \\ \hline
\textbf{CRUXEval} &
  800 &
  \multicolumn{1}{c|}{41.50\%} &
  \multicolumn{1}{c|}{58.88\%} &
  \multicolumn{1}{c|}{52.00\%} &
  \multicolumn{1}{c|}{53.00} &
  \multicolumn{1}{c|}{74.44\%} &
  86.63\% \\ \hline
\textbf{HumanEval} &
  164 &
  \multicolumn{1}{c|}{50.00\%} &
  \multicolumn{1}{c|}{64.81\%} &
  \multicolumn{1}{c|}{64.81\%} &
  \multicolumn{1}{c|}{46.60\%} &
  \multicolumn{1}{c|}{83.33\%} &
  93.21\% \\ \hline
\textbf{Total} &
  1450 &
  \multicolumn{1}{c|}{41.93\%} &
  \multicolumn{1}{c|}{60.23\%} &
  \multicolumn{1}{c|}{55.19\%} &
  \multicolumn{1}{c|}{51.11\%} &
  \multicolumn{1}{c|}{74.15\%} &
  81.17\% \\ \hline
\end{tabular}
}
\end{table}
